Determination of Black Hole Masses in Galactic Black Hole Binaries using Scaling of Spectral and Variability Characteristics

We present a study of correlations between X-ray spectral and timing properties observed from a number of Galactic Black Hole (BH) binaries during hard-soft state spectral evolution. We analyze 17 transition episodes from 8 BH sources observed with RXTE. Our scaling technique for BH mass determination uses a correlation between spectral index and quasi-periodic oscillation (QPO) frequency. In addition, we use a correlation between index and the normalization of the disk "seed" component to cross-check the BH mass determination and estimate the distance to the source. While the index-QPO correlations for two given sources contain information on the ratio of the BH masses in those sources, the index-normalization correlations depend on the ratio of the BH masses and the distance square ratio. In fact, the index-normalization correlation also discloses the index-mass accretion rate saturation effect given that the normalization of disk "seed" photon supply is proportional to the disk mass accretion rate. We present arguments that this observationally established index saturation effect is a signature of the bulk motion (converging) flow onto black hole which was early predicted by the dynamical Comptonization theory. We use GRO J1655-40 as a primary reference source for which the BH mass, distance and inclination angle are evaluated by dynamical measurements with unprecedented precision among other Galactic BH sources. We apply our scaling technique to determine BH masses and distances forCygnus X-1, GX 339-4, 4U 1543-47, XTE J1550-564, XTE J1650-500, H 1743-322 and XTE J1859-226. Good agreement of our results for sources with known values of BH masses and distance provides an independent verification for our scaling technique.

==> tab2.tex <==
J1655-R05 & 90058-16-02-00 & 53422.89 &LHS&    0.053(3) &     0.49(3) &      0.4(1) &      0.5(3) &   0.0023(1) &- & -&    0.043(2) &     0.66 \\
 & 90058-16-03-00 & 53424.01 &HSS& - &     0.53(2) &     0.70(6) & $   7.999^f$ &   0.0023(1) &- & -&    0.044(1) &     0.63 \\
 & 90058-16-04-00 & 53425.05 &LHS& - &     0.44(2) &     0.73(6) &     0.67(4) &   0.0035(2) &- & -&    0.055(1) &     0.71 \\
 & 90058-16-05-00 & 53427.02 &LHS&    0.103(2) &     0.43(2) &     0.74(6) &     0.79(7) &   0.0051(4) &- & -&    0.083(2) &     0.63 \\
 & 90058-16-06-00 & 53431.17 &LHS& - &     0.41(2) &     0.67(6) &     0.66(4) &   0.0054(3) &- & -&    0.087(2) &     0.54 \\
 & 90058-16-07-00 & 53427.94 &LHS&    0.118(3) &     0.40(1) &     0.65(5) &     0.63(3) &   0.0057(2) &- & -&    0.093(1) &     0.46 \\
 & 90428-01-01-00 & 53426.04 &LHS&    0.083(4) &     0.43(1) &     0.60(4) &     0.59(3) &   0.0041(1) &- & -&    0.069(1) &     0.65 \\
 & 90428-01-01-01 & 53427.15 &LHS&    0.109(5) &     0.42(2) &     0.69(6) &     0.69(4) &   0.0053(3) &- & -&    0.086(1) &     0.61 \\
 & 90428-01-01-02 & 53429.71 &LHS&     0.12(1) &    0.421(9) &     0.66(4) &     0.64(2) &   0.0058(2) &- & -&   0.0950(9) &     0.63 \\
 & 90428-01-01-03 & 53428.14 &LHS&    0.113(5) &     0.40(2) &     0.71(5) &     0.65(3) &   0.0059(3) &- & -&    0.092(1) &     0.76 \\
 & 90428-01-01-04 & 53428.86 &LHS&    0.121(3) &    0.396(8) &     0.72(6) &     0.90(5) &   0.0056(3) &- & -&    0.093(2) &     0.52 \\
 & 90428-01-01-05 & 53430.96 &LHS&    0.111(4) &     0.41(1) &     0.69(5) &     0.67(3) &   0.0054(2) &- & -&    0.087(1) &     0.59 \\
 & 90428-01-01-06 & 53431.61 &LHS&    0.123(4) &     0.40(2) &     0.70(6) &     0.64(3) &   0.0056(3) &- & -&    0.087(1) &     0.87 \\
 & 90428-01-01-07 & 53431.74 &LHS&    0.121(6) &     0.37(1) &     0.74(8) &     0.86(5) &   0.0053(4) &- & -&    0.085(2) &     0.48 \\
 & 90428-01-01-08 & 53431.81 &LHS&    0.121(6) &     0.42(2) &     0.79(9) &      0.9(1) &   0.0054(5) &- & -&    0.086(2) &     0.73 \\
 & 90428-01-01-09 & 53431.87 &LHS&    0.119(3) &    0.416(9) &     0.67(7) &     0.82(4) &   0.0052(3) &- & -&    0.089(2) &     0.60 \\
 & 90428-01-01-10 & 53432.79 &LHS&    0.164(3) &     0.41(1) &     0.67(5) &     0.65(2) &   0.0066(3) &- & -&   0.1073(8) &     0.58 \\
 & 91404-01-01-00 & 53433.00 &LHS&    0.163(7) &     0.40(1) &     0.66(5) &     0.63(3) &   0.0069(3) &- & -&   0.1115(7) &     0.84 \\
 & 91404-01-01-01 & 53435.61 &LHS&    0.378(7) &     0.40(1) &     0.69(4) &     0.53(2) &   0.0151(4) &- & -&   0.2295(6) &     0.68 \\
 & 91404-01-01-02 & 53433.90 &LHS&    0.243(4) &    0.394(8) &     0.70(3) &     0.60(2) &   0.0097(3) &- & -&   0.1495(3) &     0.67 \\
 & 91404-01-01-03 & 53434.69 &LHS&    0.311(8) &     0.39(1) &     0.81(7) &     0.84(6) &   0.0114(7) &- & -&   0.1745(6) &     0.58 \\
 & 91404-01-01-04 & 53436.16 &LHS&     0.41(1) &     0.43(1) &     0.60(3) &     0.43(3) &   0.0171(3) &- & -&    0.266(1) &     0.69 \\
 & 91404-01-01-05 & 53436.40 &LHS&    0.466(9) &     0.40(1) &     0.66(4) &     0.45(3) &   0.0195(5) &- & -&   0.2934(8) &     0.65 \\
 & 91702-01-01-00 & 53436.72 &LHS&    0.486(5) &    0.434(6) &     0.64(3) &     0.44(2) &   0.0212(3) &- & -&   0.3241(9) &     0.66 \\
 & 91702-01-01-01 & 53437.07 &LHS&    0.508(8) &    0.439(9) &     0.66(4) &     0.53(3) &   0.0221(6) &- & -&    0.347(1) &     0.66 \\
 & 91702-01-01-02 & 53437.14 &LHS&    0.520(7) &     0.43(1) &     0.64(3) &     0.44(2) &   0.0231(4) &- & -&    0.353(1) &     0.66 \\
 & 91702-01-01-03 & 53438.05 &LHS&    0.894(7) &    0.510(8) &     0.65(3) &     0.38(2) &   0.0343(4) &- & -&    0.502(1) &     0.51 \\
 & 91702-01-01-04 & 53438.76 &LHS&    1.352(6) &    0.566(5) &     0.62(2) &     0.32(2) &   0.0451(3) &- & -&    0.639(2) &     0.95 \\
 & 91702-01-01-05 & 53439.11 &LHS&    1.531(8) &     0.57(1) &     0.65(2) &     0.31(2) &   0.0503(5) &- & -&    0.701(3) &     0.68 \\
 & 90704-04-01-00 & 53439.74 &LHS&    2.319(6) &    0.644(9) &     0.68(2) &     0.26(1) &   0.0628(5) &- & -&    0.817(2) &     1.02 \\
 & 90704-04-01-01 & 53439.61 &LHS&    2.047(6) &    0.615(9) &     0.66(2) &     0.27(2) &   0.0585(5) &- & -&    0.779(2) &     0.79 \\
 & 91702-01-02-00G & 53440.68 &IS&      6.5(2) &    1.171(3) &    0.647(8) &     -0.2(1) &   0.2964(9) &- & -&    2.125(8) &     0.59 \\
 & 91702-01-02-01 & 53441.51 &IS&     16.7(7) &     1.22(2) &     0.69(1) &    -0.66(1) &    0.322(5) &- & -&    1.597(5) &     0.80 \\
 & 91702-01-02-02 & 53441.58 &IS&       17(3) &     1.20(3) &     0.70(1) &    -0.78(2) &    0.331(5) &- & -&    1.567(4) &     1.02 \\
 & 91702-01-02-03 & 53441.98 &IS& - &     1.19(3) &     0.72(1) &    -0.89(2) &    0.345(5) &- & -&    1.566(5) &     1.18 \\
 & 91702-01-02-04 & 53442.05 &IS& - &    1.254(4) &    0.700(2) &    -0.79(1) &    0.364(1) &- & -&    1.678(4) &     1.26 \\
 & 91702-01-02-05 & 53442.12 &IS& - &     1.19(3) &     0.72(1) &    -0.90(2) &    0.374(5) &- & -&    1.694(5) &     1.25 \\
 & 91702-01-02-06 & 53442.58 &IS& - &     1.25(2) &     0.74(1) &    -0.87(1) &    0.392(5) &- & -&    1.822(5) &     1.42 \\
\hline
J1655-D05 & 91702-01-76-03 & 53624.59 &HSS& - &     1.02(3) &    0.585(5) &    -1.28(3) &    0.102(2) &- & -&   0.2647(9) &     1.24 \\
 & 91702-01-74-02 & 53625.12 &HSS& - &     0.94(3) &      0.5(3) &    -1.24(2) &    0.098(1) &- & -&    0.269(1) &     1.46 \\
 & 91702-01-75-00 & 53626.23 &HSS& - &     0.90(3) &    0.561(5) &    -1.36(2) &    0.095(2) &- & -&   0.2282(8) &     1.18 \\
 & 91702-01-75-03 & 53626.42 &HSS& - &     0.93(5) &    0.556(6) &    -1.34(2) &    0.095(2) &- & -&   0.2272(8) &     0.61 \\
 & 91702-01-76-02 & 53627.47 &HSS& - &     0.90(2) &    0.565(4) &    -1.06(1) &    0.090(1) &- & -&   0.2752(7) &     0.91 \\
 & 91702-01-71-02 & 53627.93 &IS& - &     1.04(3) &    0.553(7) &    -0.88(2) &    0.088(2) &- & -&    0.288(1) &     1.41 \\
 & 91702-01-76-00 & 53628.20 &IS&     13.2(2) &     0.97(1) &    0.615(8) &    -0.60(1) &    0.067(1) &- & -&   0.3350(7) &     1.07 \\
 & 91702-01-76-01 & 53628.59 &IS&     12.7(1) &     1.02(3) &     0.62(1) &    -0.43(2) &    0.059(1) &- & -&    0.340(1) &     1.11 \\
 & 91702-01-71-03 & 53628.92 &IS&     9.86(4) &     0.96(2) &     0.63(2) &    -0.19(2) &    0.046(1) &- & -&    0.358(1) &     1.19 \\
 & 91702-01-71-04 & 53628.98 &IS&    10.44(5) &     0.98(2) &     0.62(1) &    -0.24(2) &    0.049(1) &- & -&    0.358(1) &     1.11 \\
 & 91702-01-79-01 & 53629.38 &IS&     9.74(3) &     0.96(2) &     0.63(1) &    -0.17(2) &    0.045(1) &- & -&    0.353(1) &     1.28 \\
 & 91702-01-79-00 & 53630.49 &IS&     8.67(1) &    0.865(9) &     0.60(1) &    -0.22(2) &   0.0411(9) &- & -&   0.3252(6) &     1.18 \\
 & 91702-01-80-00 & 53631.47 &IS&     7.81(1) &    0.810(8) &     0.65(1) &    -0.07(1) &   0.0315(5) &- & -&   0.2967(7) &     1.41 \\
 & 91702-01-80-01 & 53632.45 &LHS&     4.74(2) &    0.698(9) &     0.65(2) &     0.13(2) &   0.0230(3) &- & -&   0.2684(5) &     0.76 \\
 & 91702-01-81-00 & 53633.50 &LHS&     2.23(2) &    0.568(9) &     0.64(3) &     0.25(3) &   0.0167(2) &- & -&   0.2254(5) &     0.60 \\
 & 91702-01-80-02 & 53634.11 &LHS&     1.45(3) &     0.50(2) &     0.62(4) &     0.28(4) &   0.0141(2) &- & -&   0.1988(7) &     0.76 \\
 & 91702-01-81-01 & 53634.31 &LHS&     1.33(2) &     0.54(1) &     0.62(4) &     0.35(4) &   0.0130(2) &- & -&   0.1887(7) &     0.53 \\
 & 91702-01-81-02 & 53635.47 &LHS&    0.587(8) &     0.45(1) &     0.63(4) &     0.36(4) &   0.0094(1) &- & -&   0.1383(4) &     0.70 \\
 & 91702-01-87-03 & 53636.19 &LHS&     0.44(1) &     0.42(2) &     0.74(4) &     0.45(2) &   0.0082(2) &- & -&   0.1171(6) &     0.64 \\
 & 91702-01-82-00 & 53636.45 &LHS&    0.406(4) &     0.40(1) &      0.4(2) &      0.9(4) &   0.0049(7) &- & -&    0.102(5) &     0.78 \\
 & 91702-01-86-00 & 53638.35 &LHS&    0.227(6) &     0.46(1) &     0.54(6) &      0.3(1) &   0.0050(2) &- & -&   0.0784(8) &     0.61 \\
 & 91702-01-86-01 & 53639.14 &LHS&    0.210(7) &     0.46(2) &     0.59(6) &     0.39(7) &   0.0045(1) &- & -&   0.0694(7) &     0.66 \\
 & 91702-01-86-04 & 53639.20 &LHS&    0.206(6) &     0.49(2) &      0.5(1) &      0.6(1) &   0.0040(2) &- & -&    0.068(1) &     0.74 \\
 & 91702-01-87-00 & 53640.25 &LHS& - &     0.48(2) &     0.57(6) &     0.39(9) &  0.00373(9) &- & -&   0.0579(8) &     0.61 \\
\hline
J1550-R98 & 30188-06-01-00 & 51065.07 &LHS&    0.289(-2) &     0.57(1) &     0.64(4) &     0.70(4) &    0.162(5) &     20.3(4) &       47(1) &    2.648(4) &     1.51 \\
 & 30188-06-01-01 & 51065.34 &LHS&    0.395(3) &     0.61(1) &     0.58(5) &     0.74(5) &    0.152(5) &     19.5(4) &       45(1) &    2.542(5) &     0.51 \\
 & 30188-06-01-02 & 51066.07 &IS&    0.810(4) &     0.77(1) &     0.53(7) &      0.8(1) &    0.184(8) &     18.9(4) &     40.6(8) &    2.941(7) &     0.78 \\
 & 30188-06-01-03 & 51066.34 &IS&    1.036(4) &     0.84(1) &     0.53(9) &      1.3(-5) &     0.18(1) &     18.8(3) &     39.2(7) &      3.0(2) &     0.92 \\
 & 30188-06-02-00 & 51063.67 &LHS&   0.0630(9) &     0.36(2) &     0.75(4) &     0.66(3) &    0.085(4) &       22(5) & $     110\pm30$ &    1.267(2) &     0.62 \\
 & 30188-06-03-00 & 51064.01 &LHS&    0.116(2) &     0.40(1) &     0.71(3) &     0.62(2) &    0.101(3) &     21.8(7) &       74(2) &    1.555(2) &     0.73 \\
 & 30188-06-04-00 & 51067.27 &IS&    1.541(5) &     0.98(1) &     0.42(7) &      0.6(1) &     0.28(2) &     18.1(3) &     40.8(8) &     3.50(2) &     0.82 \\
 & 30188-06-05-00 & 51068.34 &IS&    2.392(7) &     1.16(1) &     0.49(4) &     0.40(4) &     0.37(1) &     17.9(4) &       41(1) &    3.626(9) &     0.88 \\
 & 30188-06-06-00 & 51069.27 &IS&    3.341(5) &     1.31(1) &     0.52(2) &     0.24(3) &     0.49(1) &     18.1(4) &       43(1) &    3.888(7) &     0.77 \\
 & 30188-06-07-00 & 51070.13 &IS&    3.194(4) &     1.30(1) &     0.51(2) &     0.27(3) &     0.49(1) &     18.3(4) &     41.5(9) &     3.93(1) &     1.04 \\
 & 30188-06-08-00 & 51070.27 &IS&    3.178(4) &     1.30(1) &     0.52(3) &     0.28(3) &     0.48(1) &     18.3(4) &       41(1) &    3.931(7) &     0.75 \\
 & 30188-06-09-00 & 51071.20 &IS&    3.687(5) &     1.37(1) &     0.52(2) &     0.23(3) &     0.56(1) &     18.1(4) &       45(1) &    4.224(9) &     0.84 \\
 & 30188-06-10-00 & 51072.00 &IS&    2.586(6) &     1.22(1) &     0.47(3) &     0.34(5) &     0.44(2) &     17.9(4) &       40(1) &     3.82(1) &     0.56 \\
 & 30188-06-11-00 & 51072.34 &IS&    4.035(8) &     1.42(1) &     0.55(2) &     0.22(3) &     0.59(1) &     18.1(5) &       47(1) &    4.329(9) &     0.78 \\
 & 30191-01-01-00 & 51074.14 &IS&     5.77(1) &     1.58(1) &     0.59(2) &     0.19(2) &     0.80(1) &     19.1(5) &       57(2) &     5.38(1) &     0.73 \\
 & 30191-01-02-00 & 51076.00 &HSS&     13.1(1) &     1.82(1) &     0.60(1) &      8.0\tablenotemark{f} &     1.86(2) &     20.0\tablenotemark{f} &       81(5) &    15.36(3) &     1.82 \\
 & 30191-01-03-00 & 51076.80 &IS&     7.10(2) &     1.68(1) &     0.59(2) &     0.20(3) &     1.03(2) &     20.2(6) &       61(3) &     6.57(2) &     0.96 \\
 & 30191-01-04-00 & 51076.95 &IS&     8.28(2) &     1.73(1) &     0.58(2) &     0.30(3) &     1.15(2) &     21.2(6) &       69(3) &     7.46(1) &     1.82 \\
 & 30191-01-05-00 & 51077.14 &IS&     9.95(2) &    1.838(5) &     0.53(3) &     0.57(8) &     1.28(3) &     36.8(8) &       27(3) &     8.28(3) &     1.14 \\
 & 30191-01-06-00 & 51077.21 &IS&     9.13(1) &     1.72(1) &     0.59(2) &     0.29(3) &     1.09(2) &     20.8(6) &       74(3) &     7.21(1) &     1.13 \\
 & 30191-01-08-00 & 51078.13 &IS&    5.422(9) &     1.56(1) &     0.58(2) &     0.17(2) &     0.75(1) &     19.3(5) &       53(2) &    5.021(9) &     0.82 \\
 & 30191-01-09-00 & 51079.79 &IS&     4.35(2) &     1.45(1) &     0.55(3) &     0.17(3) &     0.62(2) &     18.9(5) &       45(2) &     4.31(1) &     0.65 \\
 & 30191-01-09-01 & 51079.86 &IS&     3.97(1) &     1.41(1) &     0.53(3) &     0.17(3) &     0.60(3) &     18.7(5) &       47(2) &     4.19(1) &     0.50 \\
 & 30191-01-09-02 & 51079.93 &IS&     3.90(1) &     1.39(1) &     0.53(3) &     0.17(3) &     0.58(2) &     18.1(5) &       48(2) &     4.13(1) &     0.68 \\
 & 30191-01-10-00 & 51080.08 &IS&    3.884(6) &     1.39(1) &     0.56(3) &     0.27(3) &     0.52(2) &     18.6(4) &       45(1) &     4.11(1) &     1.03 \\
 & 30191-01-11-00 & 51081.06 &IS&    2.854(6) &     1.25(1) &     0.52(4) &     0.40(5) &     0.40(2) &     18.5(4) &     40.7(9) &     3.78(1) &     0.99 \\
 & 30191-01-12-00 & 51082.00 &IS&    2.704(6) &     1.23(1) &     0.50(5) &     0.43(6) &     0.39(2) &     18.8(4) &     40.0(8) &     3.73(2) &     0.89 \\
 & 30191-01-13-00 & 51083.00 &IS&    2.656(8) &     1.21(1) &     0.51(5) &     0.44(5) &     0.37(2) &     18.6(4) &     41.0(9) &     3.64(1) &     0.81 \\
 & 30191-01-14-00 & 51084.34 &IS&    2.688(6) &     1.20(1) &     0.53(4) &     0.42(5) &     0.36(1) &     18.8(4) &     40.2(9) &     3.57(1) &     1.32 \\
 & 30191-01-15-00 & 51085.22 &IS&    4.128(8) &     1.37(1) &     0.59(3) &     0.22(3) &     0.48(1) &     19.0(5) &       51(1) &     3.87(1) &     0.66 \\
 & 30191-01-16-00 & 51085.98 &IS&    2.988(9) &     1.23(1) &     0.55(3) &     0.32(3) &     0.38(1) &     18.8(4) &       44(1) &     3.49(1) &     0.80 \\
 & 30191-01-16-01 & 51085.90 &IS&    2.885(9) &     1.20(1) &     0.55(4) &     0.38(4) &     0.36(1) &     18.3(4) &       43(2) &     3.53(1) &     0.43 \\
 & 30191-01-17-00 & 51086.89 &IS&     3.51(1) &     1.29(1) &     0.57(3) &     0.26(3) &     0.41(1) &     19.4(4) &       45(1) &    3.540(8) &     1.42 \\
 & 30191-01-18-00 & 51087.72 &IS&    3.448(4) &     1.27(1) &     0.57(3) &     0.26(3) &     0.40(1) &     19.1(4) &       46(1) &    3.470(7) &     1.10 \\
 & 30191-01-19-00 & 51088.00 &IS&    3.232(8) &     1.25(1) &     0.57(3) &     0.29(3) &     0.38(1) &     19.3(4) &       46(1) &    3.420(9) &     0.83 \\
 & 30191-01-19-01 & 51088.07 &IS&    3.192(9) &     1.24(1) &     0.56(3) &     0.30(3) &     0.37(1) &     19.2(4) &       46(1) &    3.418(8) &     0.94 \\
 & 30191-01-20-00 & 51088.99 &IS&    3.030(8) &     1.20(1) &     0.57(3) &     0.30(3) &    0.351(9) &     19.2(4) &       44(1) &    3.291(9) &     0.83 \\
 & 30191-01-21-00 & 51090.14 &IS&     3.94(1) &     1.30(1) &     0.60(3) &     0.19(2) &    0.410(9) &     19.3(5) &       51(2) &    3.416(7) &     0.70 \\
 & 30191-01-22-00 & 51090.70 &IS&     3.76(1) &     1.28(1) &     0.58(3) &     0.20(2) &     0.39(1) &     19.3(5) &       52(2) &    3.285(8) &     1.10 \\
 & 30191-01-23-00 & 51091.74 &IS&     5.60(1) &     1.42(1) &     0.65(2) &     0.07(2) &    0.520(9) &     19.9(6) &       62(3) &    3.846(9) &     0.96 \\
 & 30191-01-24-00 & 51093.14 &IS&     6.55(1) &     1.48(1) &     0.68(2) &     0.04(2) &    0.575(8) &     21.2(9) &       90(5) &    4.155(9) &     0.64 \\
 & 30191-01-25-00 & 51094.14 &IS&    4.326(9) &     1.30(1) &     0.62(2) &     0.13(2) &    0.394(8) &     20.0(5) &       58(2) &    3.206(6) &     0.55 \\
 & 30191-01-26-00 & 51094.57 &IS&     4.99(1) &     1.35(1) &     0.65(2) &     0.07(2) &    0.433(8) &     20.1(6) &       66(3) &    3.334(7) &     1.10 \\
 & 30191-01-27-00 & 51096.57 &IS&     5.03(1) &     1.37(1) &     0.66(2) &     0.04(2) &    0.431(7) &     21.3(7) &       69(3) &    3.243(7) &     0.90 \\
 & 30191-01-27-01 & 51095.61 &IS&     4.48(1) &     1.30(1) &     0.63(2) &     0.11(2) &    0.386(7) &     21.2(6) &       56(3) &    3.105(7) &     0.82 \\
 & 30191-01-28-00 & 51097.81 &IS&     4.20(1) &     1.24(1) &     0.64(2) &     0.11(2) &    0.335(6) &     20.7(7) &       62(4) &    2.816(6) &     0.66 \\
 & 30191-01-28-01 & 51097.57 &IS&     4.74(1) &     1.30(1) &     0.64(2) &     0.07(2) &    0.375(7) &     20.3(7) &       75(5) &    2.948(6) &     0.67 \\
 & 30191-01-28-02 & 51098.27 &IS&     4.99(1) &     1.30(1) &     0.67(2) &     0.06(2) &    0.372(6) &     20.2(7) &       71(4) &    2.956(5) &     0.58 \\
 & 30191-01-29-00 & 51099.21 &IS&     4.87(1) &     1.29(1) &     0.66(2) &     0.06(2) &    0.360(6) &     20.1(7) &       71(4) &    2.865(6) &     0.60 \\
 & 30191-01-29-01 & 51099.61 &IS&     5.05(1) &     1.29(1) &     0.65(2) &     0.05(2) &    0.358(6) &     21.3(8) &       67(4) &    2.822(6) &     0.90 \\
 & 30191-01-30-00 & 51100.27 &IS&     6.49(1) &     1.39(1) &     0.69(1) &    -0.04(1) &    0.445(5) &     22.5(9) &       97(7) &    3.225(7) &     0.81 \\
 & 30191-01-31-00 & 51101.61 &IS&     6.84(2) &     1.38(1) &     0.71(1) &    -0.07(1) &    0.439(5) &       24(1) &       68(8) &    3.148(7) &     0.93 \\
 & 30191-01-31-01 & 51101.94 &IS&     6.76(2) &     1.36(1) &     0.71(1) &    -0.08(1) &    0.429(5) &     21.6(8) &       80(5) &    3.096(7) &     0.99 \\
\hline
J1550-R00 & 50137-02-01-00 & 51644.47 &LHS&    0.239(3) &    0.421(8) &     0.72(6) &     0.66(3) &    0.042(2) &       36(2) & $      60\pm10$ &    0.663(1) &     0.44 \\
 & 50137-02-02-00 & 51646.33 &LHS&    0.260(3) &     0.41(1) &     0.74(5) &     0.60(2) &    0.050(2) &       36(2) & $      40\pm10$ &    0.761(2) &     0.63 \\
 & 50137-02-02-01 & 51646.61 &LHS&    0.261(3) &    0.428(9) &     0.77(5) &     0.63(2) &    0.051(2) &       29(4) & $      90\pm30$ &    0.776(1) &     0.46 \\
 & 50137-02-03-00 & 51648.74 &LHS&    0.237(2) &     0.43(1) &     0.77(6) &     0.64(2) &    0.055(2) &       31(5) & $      80\pm40$ &    0.834(1) &     0.55 \\
 & 50137-02-03-01G & 51649.75 &LHS& - &    0.427(9) &     0.78(5) &     0.64(2) &    0.056(2) &       36(2) & $      40\pm10$ &    0.849(2) &     0.61 \\
 & 50137-02-04-00 & 51650.73 &LHS&    0.232(4) &     0.42(1) &     0.74(5) &     0.62(3) &    0.057(2) &       36(4) & $      40\pm20$ &    0.882(2) &     0.66 \\
 & 50137-02-04-01 & 51651.38 &LHS&    0.248(5) &    0.448(7) &     0.72(6) &     0.64(3) &    0.057(2) &       34(1) & $      60\pm10$ &    0.900(2) &     0.71 \\
 & 50137-02-05-00 & 51652.25 &LHS&     0.30(2) &    0.434(9) &     0.74(5) &     0.60(2) &    0.062(2) &       37(1) &       30(6) &    0.952(2) &     0.58 \\
 & 50137-02-05-01 & 51653.53 &LHS&    0.313(4) &    0.464(8) &     0.73(5) &     0.60(2) &    0.064(2) &       35(2) & $      40\pm10$ &    1.007(2) &     0.51 \\
 & 50137-02-06-00 & 51654.72 &LHS&    0.319(3) &    0.475(7) &     0.74(6) &     0.63(2) &    0.068(2) &       33(3) & $      50\pm10$ &    1.058(2) &     0.87 \\
 & 50137-02-07-00 & 51655.66 &LHS&     0.41(1) &    0.494(9) &     0.75(5) &     0.62(2) &    0.069(2) &       36(1) &       34(7) &    1.072(2) &     0.82 \\
 & 50134-02-01-00 & 51658.60 &LHS&    1.261(9) &    0.675(8) &     0.69(3) &     0.49(2) &    0.080(1) &       33(2) &       37(7) &    1.164(2) &     0.93 \\
 & 50134-02-01-01 & 51660.06 &IS&    3.999(7) &    1.021(9) &     0.64(1) &     0.02(1) &    0.131(1) &       26(1) &       59(7) &    1.198(2) &     1.17 \\
 & 50134-02-02-00 & 51662.17 &IS& - &     1.26(2) &     0.74(1) &    -0.31(1) &    0.316(4) &       33(4) & $      30\pm20$ &    2.074(4) &     1.20 \\
 & 50134-02-02-01 & 51664.41 &IS& - &     1.22(1) &    0.713(5) &   -0.634(7) &    0.269(3) &       29(3) & $      30\pm10$ &    1.353(5) &     1.78 \\
 & 50134-02-03-00 & 51664.64 &IS& - &     1.17(1) &    0.624(4) &   -0.644(7) &    0.289(3) &       34(2) &       40(9) &    1.439(7) &     0.65 \\
 & 50134-02-03-01 & 51665.40 &IS& - &     1.01(3) &     0.97(1) &    -0.46(1) &    0.125(3) &       22(1) &       43(5) &    1.123(3) &     0.68 \\
 & 50134-02-04-00 & 51667.70 &IS&      9.5(4) &     1.14(1) &    0.681(5) &   -0.723(8) &    0.208(2) &       36(3) & $      40\pm30$ &    0.957(3) &     2.04 \\
 & 50134-02-04-01 & 51668.83 &IS&      9.2(3) &     1.13(1) &    0.673(5) &   -0.751(8) &    0.197(2) &       36(2) & $      20\pm10$ &    0.877(2) &     1.76 \\
 & 50134-02-05-00 & 51669.19 &IS&      8.5(5) &     1.13(1) &    0.663(5) &   -0.790(7) &    0.198(2) &       32(3) & $      20\pm10$ &    0.838(2) &     1.68 \\
 & 50134-02-06-00 & 51670.54 &IS&      9.4(5) &     1.13(1) &    0.668(5) &   -0.657(8) &    0.173(2) &       24(3) & $     190\pm80$ &    0.824(2) &     1.67 \\
 & 50134-02-07-00 & 51670.75 &IS&      9.1(2) &     1.12(1) &    0.663(5) &   -0.757(8) &    0.178(2) &       34(4) & $      30\pm20$ &    0.778(2) &     1.88 \\
 & 50134-02-07-01 & 51671.41 &IS&      8.8(4) &     1.12(2) &    0.653(5) &   -0.782(9) &    0.175(2) &       29(6) & $      70\pm70$ &    0.737(2) &     1.71 \\
 & 50134-02-08-00 & 51672.41 &IS&      8.9(2) &     1.14(1) &    0.651(5) &   -0.694(8) &    0.158(2) &       29(6) & $      70\pm70$ &    0.708(2) &     1.83 \\
 & 50134-02-08-01 & 51672.96 &IS& - &     1.21(1) &    0.677(6) &   -0.485(8) &    0.178(2) &       29(6) & $      70\pm70$ &    0.967(2) &     1.52 \\
\hline
J1550-D00 & 50134-02-01-00 & 51658.60 &LHS&    1.261(9) &    0.675(8) &     0.69(3) &     0.49(2) &    0.080(1) &       33(2) &       37(7) &    1.164(2) &     0.93 \\
 & 50134-02-01-01 & 51660.06 &IS&    3.999(7) &    1.021(9) &     0.64(1) &     0.02(1) &    0.131(1) &       26(1) &       59(7) &    1.198(2) &     1.17 \\
 & 50134-02-02-00 & 51662.17 &IS&     4.53(2) &     1.26(1) &    0.741(8) &   -0.301(8) &    0.316(3) &       34(2) &       29(8) &    2.074(4) &     1.20 \\
 & 50134-02-02-01 & 51664.41 &IS& - &     1.22(1) &    0.713(5) &   -0.634(7) &    0.269(3) &       29(3) &       35(13) &    1.353(5) &     1.78 \\
 & 50134-02-03-00 & 51664.64 &IS& - &     1.17(1) &    0.624(4) &   -0.644(7) &    0.289(3) &       34(2) &       40(9) &    1.439(7) &     0.65 \\
 & 50134-02-03-01 & 51665.40 &IS& - &     1.01(3) &     0.97(1) &    -0.46(1) &    0.125(3) &       22(1) &       43(5) &    1.123(3) &     0.68 \\
 & 50134-02-04-00 & 51667.70 &IS&      9.5(4) &     1.14(1) &    0.681(5) &   -0.723(8) &    0.208(2) &       36(3) &       46(29) &    0.957(3) &     2.04 \\
 & 50134-02-04-01 & 51668.83 &IS&      9.2(3) &     1.13(1) &    0.673(5) &   -0.751(8) &    0.197(2) &       36(2) &       24(11) &    0.877(2) &     1.76 \\
 & 50134-02-05-00 & 51669.19 &IS&      8.5(5) &     1.13(1) &    0.663(5) &   -0.790(7) &    0.198(2) &       32(3) &       29(11) &    0.838(2) &     1.68 \\
 & 50134-02-06-00 & 51670.54 &IS&      9.4(5) &     1.13(1) &    0.668(5) &   -0.657(8) &    0.173(2) &       24(3) &      197(76) &    0.824(2) &     1.67 \\
 & 50134-02-07-00 & 51670.75 &IS&      9.1(2) &     1.12(1) &    0.663(5) &   -0.757(8) &    0.178(2) &       34(4) &       34(24) &    0.778(2) &     1.88 \\
 & 50134-02-07-01 & 51671.41 &IS&      8.8(4) &     1.12(2) &    0.653(5) &   -0.782(9) &    0.175(2) &       29(6) &       79(71) &    0.737(2) &     1.71 \\
 & 50134-02-08-00 & 51672.41 &IS&      8.9(2) &     1.14(1) &    0.651(5) &   -0.694(8) &    0.158(2) & - & - &    0.708(2) &     1.83 \\
 & 50134-02-08-01 & 51672.96 &IS& - &     1.21(1) &    0.677(6) &   -0.485(8) &    0.178(2) & - & - &    0.967(2) &     1.52 \\
 & 50134-01-01-00 & 51673.41 &IS& - &    1.169(5) &    0.594(4) &   -0.628(7) &    0.200(2) & - & - &    0.896(3) &     0.88 \\
 & 50134-01-02-00 & 51674.69 &IS& - &    1.111(5) &    0.585(6) &   -0.508(7) &    0.184(2) & - & - &    0.949(3) &     0.62 \\
 & 50134-01-03-00 & 51675.46 &IS&      7.6(1) &    1.104(3) &    0.563(9) &   -0.373(8) &    0.129(1) & - & - &    0.739(2) &     1.21 \\
 & 50134-01-04-00 & 51676.40 &IS&     6.87(2) &     1.05(1) &    0.641(8) &    -0.32(1) &    0.099(1) & - & - &    0.643(1) &     1.61 \\
 & 50134-01-05-00 & 51678.45 &IS&     4.46(2) &    0.937(8) &     0.64(1) &    -0.06(1) &   0.0668(8) & - & - &    0.589(1) &     1.13 \\
 & 50135-01-01-00 & 51680.38 &IS&     4.14(2) &    0.912(8) &     0.63(1) &     0.01(1) &   0.0559(7) & - & - &    0.528(1) &     1.07 \\
 & 50135-01-02-00 & 51682.30 &IS&     2.34(1) &    0.721(9) &     0.67(2) &     0.22(2) &   0.0375(3) & - & - &   0.4598(9) &     0.57 \\
 & 50135-01-03-00 & 51683.77 &LHS&     1.12(1) &    0.564(8) &     0.71(3) &     0.38(2) &   0.0286(3) & - & - &   0.4021(7) &     0.57 \\
 & 50135-01-04-00 & 51684.76 &LHS&     0.99(3) &     0.56(1) &     0.69(3) &     0.46(2) &   0.0246(4) & - & - &   0.3612(8) &     0.60 \\
 & 50135-01-05-00 & 51686.30 &LHS&     0.68(1) &    0.510(9) &     0.71(3) &     0.48(2) &   0.0209(4) & - & - &   0.3086(8) &     0.47 \\
 & 50135-01-06-00 & 51687.22 &LHS& - &     0.49(1) &     0.71(3) &     0.49(2) &   0.0185(4) & - & - &   0.2742(9) &     0.71 \\
 & 50135-01-07-00 & 51688.84 &LHS&    0.355(7) &     0.47(1) &     0.70(4) &     0.54(3) &   0.0141(4) & - & - &   0.2162(8) &     0.68 \\
 & 50135-01-08-00 & 51690.77 &LHS&     0.31(4) &     0.45(2) &     0.57(6) &     0.50(7) &   0.0100(3) & - & - &   0.1660(7) &     0.59 \\
 & 50135-01-08-01 & 51690.84 &LHS&     0.22(2) &     0.47(2) &     0.70(6) &     0.60(3) &   0.0107(5) & - & - &   0.1666(7) &     0.70 \\
 & 50135-01-09-00 & 51692.55 &LHS& - &     0.43(2) &     0.70(5) &     0.55(3) &   0.0081(3) & - & - &   0.1243(7) &     0.67 \\
\hline
J1650-R01 & 60113-01-03-00 & 52160.38 &LHS&     0.98(1) &    0.609(9) &     0.66(3) &     0.40(2) &    0.106(1) &       25(2) &      119(12) &    1.542(3) &     0.86 \\
 & 60113-01-04-00 & 52161.11 &LHS&     1.13(1) &    0.656(6) &     0.65(3) &     0.41(2) &    0.109(1) &       32(1) &       66(8) &    1.581(2) &     0.71 \\
 & 60113-01-05-00 & 52162.45 &LHS&     1.30(1) &    0.681(8) &     0.66(3) &     0.37(2) &    0.112(1) &       36(2) &       47(14) &    1.561(2) &     0.63 \\
 & 60113-01-05-01 & 52162.59 &IS&     1.34(1) &    0.700(8) &     0.65(3) &     0.37(2) &    0.112(1) &       34(2) &       62(13) &    1.555(3) &     0.67 \\
 & 60113-01-06-00 & 52163.44 &IS&     1.53(1) &    0.702(9) &     0.67(3) &     0.32(2) &    0.113(1) &       25(2) &      111(12) &    1.516(3) &     0.58 \\
 & 60113-01-07-00 & 52165.16 &IS&     1.90(1) &     0.74(1) &     0.65(2) &     0.21(2) &   0.1120(8) &       22(2) &      112(12) &    1.375(2) &     0.80 \\
 & 60113-01-08-00 & 52166.09 &IS&     2.35(2) &    0.820(7) &     0.63(2) &     0.17(2) &    0.113(1) &       33(2) &       52(12) &    1.316(2) &     0.78 \\
 & 60113-01-08-01 & 52166.56 &IS&     2.09(3) &     0.78(1) &     0.65(2) &     0.21(2) &   0.1108(9) &       37(2) &       35(12) &    1.332(3) &     0.56 \\
 & 60113-01-09-00 & 52167.49 &IS&     2.79(2) &     0.85(1) &     0.63(2) &     0.06(2) &    0.119(1) &       21(2) &      125(17) &    1.238(3) &     0.92 \\
 & 60113-01-09-01 & 52167.56 &IS&     2.71(2) &    0.857(9) &     0.62(2) &     0.07(1) &    0.117(1) &       28(4) &       69(23) &    1.236(2) &     0.79 \\
 & 60113-01-09-02 & 52167.62 &IS&     2.73(2) &     0.86(1) &     0.63(2) &     0.10(2) &    0.116(1) &       23(2) &       95(16) &    1.235(2) &     0.77 \\
 & 60113-01-10-00 & 52168.41 &IS&     3.04(2) &     0.88(1) &     0.63(2) &     0.03(2) &    0.119(1) &       23(2) &      111(16) &    1.185(2) &     0.69 \\
 & 60113-01-10-01 & 52168.48 &IS&     3.01(2) &    0.884(9) &     0.61(2) &     0.03(1) &    0.119(2) &       35(2) &       36(10) &    1.190(3) &     0.94 \\
 & 60113-01-11-00 & 52169.40 &IS&     3.27(2) &     0.89(1) &     0.62(2) &    -0.02(1) &    0.120(2) &       23(2) &      113(16) &    1.141(3) &     0.76 \\
 & 60113-01-11-01 & 52169.47 &IS&     3.35(2) &     0.92(1) &     0.60(1) &    -0.04(1) &    0.123(2) &       36(3) &       47(19) &    1.134(2) &     0.93 \\
 & 60113-01-11-02 & 52169.54 &IS&     3.56(2) &     0.92(1) &     0.61(1) &    -0.08(1) &    0.127(2) &       32(5) &       45(30) &    1.132(2) &     0.92 \\
 & 60113-01-12-00 & 52170.25 &IS&     4.09(2) &    0.966(9) &     0.59(1) &    -0.17(1) &    0.136(2) &       28(3) &       75(20) &    1.075(2) &     1.05 \\
 & 60113-01-12-01 & 52170.46 &IS&     4.36(2) &     0.98(1) &     0.60(1) &    -0.19(1) &    0.138(2) &       24(6) &      103(41) &    1.064(2) &     0.96 \\
 & 60113-01-12-02 & 52170.60 &IS&     4.84(3) &     1.02(1) &     0.59(1) &    -0.26(1) &    0.149(3) &       32(3) &       41(16) &    1.036(3) &     1.09 \\
 & 60113-01-12-03 & 52170.81 &IS&     4.64(3) &     1.05(2) &     0.57(2) &    -0.21(2) &    0.148(4) & - & - &    1.038(4) &     0.67 \\
 & 60113-01-12-04 & 52170.87 &IS&     5.16(4) &     1.05(2) &     0.57(2) &    -0.21(2) &    0.148(4) & - & - &    1.038(4) &     0.67 \\
 & 60113-01-13-00 & 52171.53 &IS&     5.77(3) &    1.102(8) &    0.583(9) &    -0.36(1) &    0.162(3) & - & - &    0.952(2) &     1.31 \\
 & 60113-01-13-01 & 52171.66 &IS&     6.32(4) &     1.07(1) &    0.590(8) &    -0.45(1) &    0.168(3) & - & - &    0.928(2) &     1.20 \\
 & 60113-01-13-02 & 52171.77 &IS&     6.87(6) &     1.11(1) &    0.576(8) &    -0.52(1) &    0.182(4) & - & - &    0.896(2) &     1.38 \\
 & 60113-01-14-00 & 52171.90 &IS& - &     1.07(1) &    0.590(6) &    -0.67(1) &    0.196(4) &       22(1) &       91(15) &    0.851(2) &     1.47 \\
 & 60113-01-14-01G & 52172.10 &IS& - &     1.07(1) &    0.591(7) &    -0.62(1) &    0.191(3) &       33(2) &       41(15) &    0.879(2) &     1.27 \\
 & 60113-01-15-00 & 52173.09 &IS& - &     1.15(2) &    0.570(5) &   -0.894(9) &    0.231(4) &       25(4) &       95(42) &    0.746(2) &     1.63 \\
 & 60113-01-16-00 & 52174.30 &HSS& - &     1.05(2) &    0.558(5) &    -1.00(1) &    0.210(4) &       37(2) &       11(8) &    0.625(2) &     1.31 \\
 & 60113-01-16-01 & 52174.77 &HSS& - &     1.05(2) &    0.558(5) &    -1.00(1) &    0.210(4) & - & - &    0.625(2) &     1.31 \\
 & 60113-01-16-02 & 52174.91 &IS& - &     1.07(2) &    0.553(5) &    -0.96(1) &    0.208(4) &       34(6) &       10(13) &    0.627(2) &     0.89 \\
 & 60113-01-17-00 & 52175.15 &IS& - &     1.12(1) &    0.563(4) &   -0.925(9) &    0.217(4) &       34(3) &       34(20) &    0.679(2) &     1.68 \\
 & 60113-01-18-00 & 52176.03 &IS& - &     1.05(2) &    0.552(5) &    -0.99(1) &    0.201(4) &       23(1) &       45(10) &    0.593(2) &     1.28 \\
 & 60113-01-18-01 & 52176.07 &IS& - &     1.06(1) &    0.554(5) &    -0.97(1) &    0.198(4) &       23(2) &       73(17) &    0.596(2) &     1.39 \\
 & 60113-01-18-02 & 52176.76 &HSS& - &     1.12(2) &    0.526(4) &    -1.21(1) &    0.217(5) & - & - &    0.475(1) &     0.98 \\
 & 60113-01-19-00 & 52177.34 &HSS& - &     1.06(2) &    0.534(4) &    -1.17(1) &    0.207(4) &       24(1) &       24(6) &    0.490(2) &     1.13 \\
 & 60113-01-19-01 & 52178.78 &HSS& - &     1.15(3) &    0.519(5) &    -1.15(2) &    0.207(5) & - & - &    0.459(2) &     0.95 \\
 & 60113-01-19-02 & 52179.71 &HSS& - &     1.15(4) &    0.511(5) &    -1.29(2) &    0.212(6) & - & - &    0.404(2) &     0.69 \\
 & 60113-01-19-03 & 52179.84 &HSS& - &     1.10(4) &    0.511(5) &    -1.26(2) &    0.211(5) & - & - &    0.422(2) &     0.82 \\
 & 60113-01-19-04 & 52179.77 &HSS& - &     1.11(4) &    0.501(4) &    -1.43(2) &    0.220(5) & - & - &    0.371(2) &     1.07 \\
 & 60113-01-19-05 & 52179.90 &HSS& - &     1.12(3) &    0.517(5) &    -1.15(2) &    0.203(5) & - & - &    0.452(2) &     1.09 \\
 & 60113-01-19-06 & 52179.97 &HSS& - &     1.19(4) &    0.498(7) &    -1.16(2) &    0.213(7) & - & - &    0.428(2) &     0.75 \\
 & 60113-01-20-00 & 52180.70 &HSS& - &     1.17(3) &    0.517(5) &    -1.04(2) &    0.195(5) & - & - &    0.469(2) &     0.92 \\
\hline
GX339-R02 & 70109-01-04-00 & 52387.55 &LHS&    0.159(1) &    0.574(9) &     0.69(3) &     0.57(2) &    0.097(2) &     25.2(8) &       64(3) &    1.531(3) &     1.11 \\
 & 40031-03-02-05 & 52388.05 &LHS&     0.19(1) &     0.55(2) &     0.68(6) &     0.53(4) &    0.099(4) &       23(2) &       64(8) &    1.548(3) &     0.68 \\
 & 40031-03-02-06 & 52389.06 &LHS& - &     0.57(2) &     0.67(7) &     0.55(5) &    0.099(4) &       21(2) &       69(10) &    1.549(4) &     0.72 \\
 & 70110-01-07-00 & 52390.90 &LHS& - &     0.56(2) &     0.70(4) &     0.53(3) &    0.103(3) &       21(1) &       74(8) &    1.578(5) &     0.65 \\
 & 70109-01-05-00 & 52391.38 &LHS&     0.22(2) &     0.58(1) &     0.70(5) &     0.57(3) &    0.100(3) &     23.0(9) &       69(3) &    1.558(3) &     1.10 \\
 & 70109-01-05-02 & 52391.45 &LHS&    0.199(1) &     0.59(1) &     0.69(4) &     0.57(3) &    0.101(2) &       24(1) &       67(4) &    1.576(3) &     0.79 \\
 & 70110-01-08-00 & 52394.44 &LHS&    0.262(6) &     0.60(1) &     0.67(3) &     0.55(2) &    0.102(2) &     22.3(8) &       73(5) &    1.586(3) &     0.58 \\
 & 70110-01-09-00 & 52398.66 &LHS&     0.21(2) &     0.66(1) &     0.69(3) &     0.55(3) &    0.105(2) &       23(1) &       69(6) &    1.581(4) &     0.52 \\
 & 70109-01-06-00 & 52400.83 &IS&    0.611(9) &     0.75(1) &     0.70(3) &     0.47(3) &    0.109(2) &     21.6(8) &       62(3) &    1.528(3) &     0.66 \\
 & 70108-03-01-00 & 52400.85 &IS&     0.61(1) &     0.78(1) &     0.66(3) &     0.50(3) &    0.107(2) &     23.2(8) &       61(2) &    1.513(3) &     1.07 \\
 & 70110-01-10-00 & 52402.49 &IS&     2.06(2) &     1.04(1) &     0.62(2) &     0.17(2) &    0.129(1) &       21(1) &       84(11) &    1.297(3) &     0.92 \\
 & 70109-04-01-00 & 52405.58 &IS&     5.37(2) &     1.35(1) &    0.654(9) &   -0.342(9) &    0.223(3) &       23(1) &       90(11) &    1.255(3) &     0.92 \\
 & 70109-04-01-01 & 52405.71 &IS&     5.35(1) &     1.35(1) &    0.657(9) &   -0.340(9) &    0.222(3) &       22(1) &       97(9) &    1.257(3) &     0.94 \\
 & 70109-04-01-02 & 52406.07 &IS&     5.34(3) &     1.37(2) &     0.62(1) &    -0.31(1) &    0.223(3) &       21(2) &      140(61) &    1.250(3) &     0.89 \\
 & 70110-01-11-00 & 52406.70 &IS&     5.79(3) &     1.39(1) &    0.650(9) &    -0.37(1) &    0.226(3) &       38(2) &       13(7) &    1.227(3) &     0.78 \\
 & 70110-01-12-00 & 52410.53 &IS&      7.9(1) &     1.40(1) &    0.657(7) &   -0.611(9) &    0.253(3) &       23(2) &       82(22) &    1.123(2) &     1.02 \\
 & 70109-01-07-00 & 52411.60 &IS&      7.1(4) &     1.52(1) &    0.677(6) &   -0.724(8) &    0.269(3) &       25(2) &       57(14) &    1.102(3) &     1.07 \\
 & 70110-01-13-00 & 52412.07 &IS& - &     1.56(3) &    0.655(6) &    -0.82(2) &    0.274(4) &       24(7) &       74(79) &      1.0(3) &     0.68 \\
\hline
GX339-D03 & 70128-02-01-01 & 52690.98 &HSS& - &      1.3(2) &    0.463(6) &     -1.7(1) &    0.057(2) &- & -&   0.0632(7) &     0.98 \\
 & 70109-01-37-00 & 52694.92 &HSS& - &     1.21(3) &    0.483(6) &    -1.08(2) &    0.043(1) &- & -&   0.0886(9) &     1.18 \\
 & 70128-02-02-00 & 52696.36 &IS&     8.07(3) &     1.05(2) &    0.515(7) &   -0.995(4) &    0.035(1) &- & -&    0.095(1) &     1.66 \\
 & 70110-01-85-00 & 52697.14 &IS& - &     1.30(5) &    0.478(7) &    -0.98(3) &    0.039(2) &- & -&   0.0835(9) &     0.98 \\
 & 70110-01-86-00 & 52697.14 &HSS& - &      1.0(1) &     0.48(1) &    -1.27(7) &    0.045(2) &- & -&    0.082(1) &     0.53 \\
 & 70110-01-87-00 & 52700.59 &HSS& - &     1.17(5) &    0.473(7) &    -1.08(3) &    0.035(1) &- & -&    0.071(1) &     0.66 \\
 & 70110-01-88-00 & 52704.01 &IS&      7.9(1) &     1.02(4) &    0.496(8) &    -0.98(2) &    0.029(1) &- & -&    0.077(1) &     1.02 \\
 & 70110-01-89-00 & 52707.91 &IS& - &     1.22(5) &    0.483(8) &    -0.99(2) &    0.033(1) &- & -&    0.075(1) &     0.94 \\
 & 50117-01-03-00 & 52706.84 &IS&     6.83(7) &     0.97(2) &     0.52(1) &    -0.76(1) &   0.0238(8) &- & -&    0.090(1) &     1.30 \\
 & 50117-01-03-01 & 52706.77 &IS&     6.72(3) &     1.02(3) &     0.51(1) &    -0.74(2) &    0.024(1) &- & -&    0.089(1) &     1.09 \\
 & 70109-02-01-00 & 52709.86 &IS&     8.08(5) &     1.11(2) &    0.488(5) &   -0.955(9) &   0.0296(8) &- & -&   0.0746(8) &     1.13 \\
 & 70109-02-01-01 & 52709.99 &IS&     8.30(5) &     1.11(3) &    0.487(6) &    -0.98(2) &   0.0300(9) &- & -&   0.0738(8) &     0.92 \\
 & 60705-01-56-00 & 52710.71 &IS&      7.7(2) &     1.08(3) &    0.503(7) &    -0.87(2) &   0.0276(9) &- & -&    0.081(1) &     0.79 \\
 & 50117-01-04-00 & 52715.84 &HSS& - &     1.08(3) &    0.461(3) &    -1.55(1) &   0.0398(9) &- & -&   0.0510(5) &     1.31 \\
 & 50117-01-04-01 & 52718.08 &HSS&      8.3(3) &     1.10(4) &    0.478(6) &    -1.11(2) &    0.034(1) &- & -&   0.0723(8) &     0.73 \\
 & 50117-01-04-02 & 52718.17 &HSS& - &     1.21(8) &     0.46(1) &    -1.08(4) &    0.036(2) &- & -&    0.070(1) &     0.85 \\
 & 60705-01-57-00 & 52716.70 &HSS& - &     1.01(5) &    0.475(5) &    -1.43(2) &    0.037(1) &- & -&   0.0588(7) &     0.60 \\
 & 60705-01-59-00 & 52731.56 &IS&     2.86(4) &     0.78(2) &     0.62(2) &    -0.02(2) &   0.0104(2) &- & -&    0.107(1) &     0.68 \\
 & 60705-01-61-00 & 52746.96 &LHS& - &     0.53(2) &     0.58(7) &     0.59(6) &   0.0032(2) &- & -&    0.055(3) &     0.75 \\
 & 60705-01-62-00 & 52750.36 &LHS&     0.29(1) &     0.50(3) &     0.63(7) &     0.60(7) &   0.0025(1) &- & -&    0.041(2) &     0.48 \\
 & 60705-01-63-00 & 52756.04 &LHS& - &     0.51(4) &     0.60(6) &     0.54(7) &  0.00158(8) &- & -&    0.026(1) &     0.59 \\
 & 60705-01-64-00 & 52765.64 &LHS& - &     0.50(5) &     0.68(9) &     0.61(9) &  0.00107(9) &- & -&    0.017(2) &     0.70 \\
 & 70109-02-02-00 & 52713.08 &HSS&      8.8(3) &     1.12(2) &    0.484(5) &    -1.09(1) &   0.0320(9) &- & -&   0.0682(7) &     0.85 \\
 & 70110-01-90-00 & 52711.51 &IS& - &     1.18(5) &    0.480(9) &    -0.84(2) &    0.030(1) &- & -&    0.082(2) &     1.04 \\
 & 70110-01-91-00 & 52713.48 &HSS& - &     1.15(7) &    0.468(8) &    -1.21(4) &    0.036(2) &- & -&   0.0627(9) &     0.76 \\
 & 70110-01-92-00 & 52717.49 &HSS& - &     0.98(9) &    0.466(6) &    -1.40(4) &    0.038(2) &- & -&   0.0608(8) &     0.68 \\
 & 70110-01-93-00 & 52719.23 &IS& - &     1.16(8) &     0.49(1) &    -0.92(4) &    0.031(1) &- & -&    0.080(1) &     0.68 \\
 & 70110-01-94-00 & 52724.22 &IS&     6.14(3) &     1.10(5) &     0.50(1) &    -0.63(3) &    0.023(1) &- & -&    0.094(2) &     0.58 \\
 & 70110-01-95-00 & 52727.25 &IS&     4.70(8) &     1.00(6) &     0.53(3) &    -0.35(5) &    0.016(1) &- & -&    0.100(3) &     0.65 \\
 & 70110-01-96-00 & 52732.11 &LHS&      2.4(4) &     0.66(5) &     0.62(5) &     0.07(5) &   0.0096(3) &- & -&    0.112(3) &     0.60 \\
 & 70110-01-97-00 & 52734.22 &IS& - &     0.70(4) &     0.58(5) &     0.19(5) &   0.0083(2) &- & -&    0.106(3) &     0.60 \\
 & 70110-01-98-00 & 52737.25 &IS&      1.8(3) &     0.70(5) &     0.60(8) &      0.4(1) &   0.0065(3) &- & -&    0.097(5) &     0.61 \\
 & 70111-01-01-00 & 52737.25 &HSS& - &      1.0(2) &    0.477(5) &    -1.85(8) &    0.053(2) &- & -&   0.0647(6) &     0.92 \\
 & 70128-02-03-00 & 52742.23 &LHS&     1.15(6) &    0.585(9) &     0.59(4) &     0.52(3) &  0.00496(9) &- & -&    0.079(2) &     1.04 \\
 & 70128-02-03-01 & 52742.61 &LHS&     1.07(6) &     0.52(1) &     0.66(3) &     0.46(2) &   0.0051(1) &- & -&    0.078(2) &     0.63 \\
 & 80116-02-01-00 & 52735.64 &LHS& - &     0.60(1) &     0.62(3) &     0.27(2) &  0.00757(7) &- & -&    0.104(1) &     0.67 \\
 & 80116-02-01-01G & 52735.64 &LHS& - &     0.58(2) &     0.65(3) &     0.34(2) &   0.0069(1) &- & -&    0.098(2) &     0.62 \\
 & 80116-02-01-02 & 52739.58 &LHS&      1.4(2) &     0.55(1) &     0.64(3) &     0.34(2) &  0.00626(9) &- & -&    0.090(1) &     0.43 \\
 & 70110-01-01-10 & 52740.01 &LHS& - &     0.64(4) &     0.47(7) &      0.2(2) &   0.0060(7) &- & -&    0.088(5) &     0.77 \\
 & 80116-02-02-00 & 52741.70 &LHS&     1.31(7) &     0.55(1) &     0.62(3) &     0.43(3) &  0.00548(9) &- & -&    0.083(1) &     0.55 \\
 & 80116-02-02-01 & 52742.04 &LHS&     1.24(4) &     0.59(2) &     0.57(5) &     0.50(5) &   0.0050(1) &- & -&    0.081(2) &     0.86 \\
 & 70110-01-02-10 & 52743.16 &LHS& - &     0.64(4) &     0.47(7) &      0.2(2) &   0.0060(7) &- & -&    0.088(5) &     0.77 \\
 & 70110-01-03-10 & 52747.40 &LHS& - &     0.51(3) &     0.57(9) &     0.53(8) &   0.0032(2) &- & -&    0.054(4) &     0.65 \\
 & 70110-01-04-10 & 52751.56 &LHS& - &     0.49(5) &      0.6(1) &      0.5(1) &   0.0022(2) &- & -&    0.037(3) &     0.46 \\
 & 70110-01-05-10 & 52756.38 &LHS& - &     0.43(7) &     0.65(7) &     0.49(9) &   0.0017(2) &- & -&    0.026(3) &     0.73 \\
 & 80102-04-01-00 & 52763.34 &LHS& - &     0.52(8) &      0.7(1) &      0.5(1) &   0.0011(1) &- & -&    0.017(2) &     0.62 \\
\hline
GX339-R04 & 60705-01-65-00 & 53198.29 &LHS&    0.306(7) &     0.45(1) &     0.66(3) &     0.50(2) &   0.0166(4) &- & -&    0.2595(7) &     0.75 \\
 & 60705-01-65-01 & 53201.32 &LHS&     0.36(1) &     0.48(1) &     0.67(4) &     0.48(3) &   0.0185(5) &- & -&     0.286(1) &     0.58 \\
 & 60705-01-66-00 & 53204.41 &LHS& - &     0.50(1) &     0.65(4) &     0.52(3) &   0.0192(5) &- & -&    0.3046(9) &     0.82 \\
 & 60705-01-66-02 & 53207.90 &LHS&     0.42(6) &     0.49(1) &     0.63(3) &     0.45(3) &   0.0209(4) &- & -&     0.324(1) &     0.82 \\
 & 60705-01-67-01 & 53215.29 &LHS& - &    0.519(9) &     0.61(3) &     0.47(3) &   0.0231(4) &- & -&    0.3666(8) &     0.72 \\
 & 60705-01-68-00 & 53218.11 &LHS&    0.461(7) &    0.519(9) &     0.61(3) &     0.47(3) &   0.0231(4) &- & -&    0.3666(8) &     0.72 \\
 & 60705-01-68-01 & 53222.24 &LHS&     1.06(2) &     0.60(1) &     0.61(4) &     0.34(4) &   0.0316(5) &- & -&     0.458(1) &     1.05 \\
 & 60705-01-69-00 & 53225.40 &LHS&     1.30(2) &     0.65(2) &     0.65(5) &     0.39(3) &   0.0330(7) &- & -&     0.474(1) &     1.12 \\
 & 60705-01-69-01 & 53228.99 &IS&     1.43(3) &     0.80(1) &     0.63(2) &     0.21(2) &   0.0367(3) &- & -&     0.444(1) &     0.93 \\
 & 60705-01-70-00 & 53230.96 &IS&     4.29(3) &     1.10(2) &     0.57(1) &    -0.34(2) &    0.060(1) &- & -&     0.369(1) &     1.15 \\
 & 60705-01-70-01 & 53234.58 &HSS& - &     1.23(8) &     0.53(2) &    -1.05(6) &    0.112(6) &- & -&     0.301(3) &     0.82 \\
 & 90110-02-01-00 & 53232.40 &IS&     5.41(3) &    1.049(4) &    0.488(7) &   -0.704(7) &   0.0900(5) &- & -&     0.352(1) &     0.59 \\
 & 90110-02-01-01 & 53232.01 &IS&     5.06(5) &     1.16(2) &    0.566(9) &    -0.44(1) &    0.069(1) &- & -&    0.3602(7) &     0.95 \\
 & 90110-02-01-02 & 53232.34 &IS&     5.21(3) &     1.11(1) &     0.52(2) &    -0.54(2) &    0.076(2) &- & -&    0.3596(9) &     1.14 \\
 & 90110-02-01-03 & 53232.99 &IS&      8.0(2) &    1.214(7) &    0.520(8) &   -0.875(5) &    0.117(2) &- & -&     0.362(1) &     0.66 \\
 & 90418-01-01-00 & 53196.21 &LHS& - &     0.50(1) &     0.65(5) &     0.53(4) &   0.0150(5) &- & -&     0.237(1) &     0.63 \\
 & 90418-01-01-01 & 53197.09 &LHS& - &    0.481(7) &     0.62(5) &     0.48(4) &   0.0157(4) &- & -&    0.2498(5) &     0.94 \\
 & 90418-01-01-02 & 53198.14 &LHS&    0.325(7) &    0.493(6) &     0.63(5) &     0.50(3) &   0.0161(4) &- & -&    0.2542(5) &     1.00 \\
 & 90418-01-01-03 & 53199.12 &LHS&    0.340(9) &    0.494(7) &     0.61(5) &     0.47(4) &   0.0170(4) &- & -&    0.2716(5) &     1.21 \\
 & 90418-01-01-04 & 53196.14 &LHS& - &     0.50(2) &     0.69(5) &     0.56(4) &   0.0150(4) &- & -&     0.235(1) &     0.87 \\
 & 90704-01-01-00 & 53226.43 &LHS&     0.73(2) &     0.64(1) &     0.61(7) &     0.33(5) &   0.0340(8) &- & -&    0.4841(8) &     1.12 \\
 & 90704-01-02-00 & 53233.39 &IS&      7.9(2) &     1.18(4) &     0.50(1) &    -0.87(5) &    0.120(5) &- & -&     0.380(2) &     0.76 \\
 & 90704-01-03-00 & 53235.43 &HSS& - &     1.20(3) &     0.50(2) &    -1.11(3) &    0.122(6) &- & -&     0.302(9) &     0.78 \\
 & 90704-01-04-00 & 53236.27 &HSS& - &     1.13(8) &     0.49(2) &    -1.33(5) &    0.117(7) &- & -&     0.228(9) &     0.71 \\
 & 90704-02-01-01 & 53237.53 &HSS& - &     1.08(3) &    0.511(4) &    -1.34(2) &    0.110(2) &- & -&    0.2275(8) &     0.95 \\
 & 90704-02-01-00 & 53237.32 &HSS& - &     1.12(2) &    0.514(4) &    -1.28(1) &    0.108(2) &- & -&    0.2339(7) &     1.19 \\
 & 90704-02-01-02 & 53237.60 &HSS& - &     1.12(4) &    0.516(5) &    -1.28(2) &    0.106(2) &- & -&    0.2300(9) &     0.70 \\
 & 90704-02-01-03 & 53237.67 &HSS& - &     1.07(4) &    0.514(5) &    -1.29(2) &    0.107(2) &- & -&    0.2328(8) &     0.85 \\
\hline
GX339-R07 & 92428-01-02-00 & 54122.27 &LHS& - &    0.455(9) &     0.61(3) &     0.39(3) &   0.0566(8) &       26(3) &       76(14) &    0.872(2) &     0.82 \\
 & 92428-01-03-00 & 54127.11 &LHS& - &     0.50(2) &     0.55(5) &     0.33(6) &    0.070(2) &       28(6) &       50(29) &    1.089(9) &     0.93 \\
 & 92035-01-01-00 & 54129.47 &LHS&    0.164(6) &     0.51(1) &     0.65(3) &     0.44(2) &    0.076(1) &       21(2) &       95(9) &    1.160(2) &     0.73 \\
 & 92035-01-01-01 & 54128.94 &LHS&    0.142(3) &    0.484(8) &     0.53(2) &     0.19(3) &    0.080(1) &       26(1) &       66(6) &    1.137(3) &     0.87 \\
 & 92035-01-01-02 & 54131.10 &LHS&    0.180(4) &    0.527(9) &     0.59(3) &     0.38(3) &   0.0834(9) &       26(1) &       67(6) &    1.276(3) &     1.03 \\
 & 92035-01-01-03 & 54130.13 &LHS&    0.167(4) &     0.48(1) &     0.55(2) &     0.20(3) &    0.086(1) &       22(1) &       73(6) &    1.214(3) &     0.86 \\
 & 92035-01-01-04 & 54132.08 &LHS&    0.200(3) &     0.53(1) &     0.59(3) &     0.39(3) &    0.085(1) &       24(1) &       71(6) &    1.314(2) &     1.03 \\
 & 92035-01-02-00 & 54133.00 &LHS&    0.237(8) &     0.55(1) &     0.58(3) &     0.39(3) &    0.088(1) &       25(4) &       72(19) &    1.354(3) &     0.90 \\
 & 92035-01-02-01 & 54133.92 &LHS&    0.264(6) &    0.554(9) &     0.59(3) &     0.37(3) &   0.0899(9) &     25.2(9) &       68(6) &    1.362(3) &     0.98 \\
 & 92035-01-02-02 & 54135.03 &LHS&    0.296(4) &    0.569(9) &     0.57(3) &     0.38(3) &    0.090(1) &     24.5(8) &       60(4) &    1.380(3) &     0.83 \\
 & 92035-01-02-03 & 54136.02 &LHS&    0.361(6) &     0.56(1) &     0.60(3) &     0.37(3) &    0.094(1) &     22.7(9) &       72(5) &    1.414(3) &     1.16 \\
 & 92035-01-02-04 & 54137.00 &LHS&    0.432(5) &     0.60(1) &     0.62(3) &     0.43(2) &    0.100(1) &     22.8(8) &       70(4) &    1.510(3) &     0.76 \\
 & 92035-01-02-08 & 54137.85 &LHS&     0.53(2) &     0.63(1) &     0.54(3) &     0.33(4) &    0.104(2) &       21(1) &       78(8) &    1.522(3) &     0.98 \\
 & 92035-01-02-06 & 54139.94 &IS&    0.987(5) &     0.79(1) &     0.61(2) &     0.36(2) &    0.111(1) &     21.9(7) &       65(3) &    1.466(2) &     0.73 \\
 & 92035-01-02-07 & 54138.83 &LHS&    0.900(5) &     0.64(1) &     0.52(2) &     0.16(3) &    0.117(2) &     21.6(7) &       68(3) &    1.521(3) &     0.78 \\
 & 92035-01-03-00 & 54140.20 &IS&    1.136(2) &     0.82(1) &     0.56(2) &     0.25(3) &    0.117(2) &     21.0(8) &       75(5) &    1.438(2) &     0.72 \\
 & 92035-01-03-01 & 54141.05 &IS&    1.691(3) &     0.92(1) &     0.55(2) &     0.15(2) &    0.131(2) &     20.6(9) &       79(6) &    1.384(3) &     0.74 \\
 & 92035-01-03-02 & 54142.04 &IS&    2.434(9) &     1.03(1) &     0.51(1) &    -0.14(2) &    0.182(5) &     20.6(8) &       72(5) &    1.343(2) &     0.85 \\
 & 92035-01-03-03 & 54143.02 &IS&    3.508(9) &     1.22(1) &     0.55(1) &    -0.17(1) &    0.208(4) &       24(1) &       67(10) &    1.338(2) &     0.91 \\
 & 92428-01-04-00 & 54143.87 &IS&     4.34(1) &     1.29(1) &    0.597(9) &    -0.25(1) &    0.226(3) &       22(1) &       80(11) &    1.337(3) &     1.00 \\
 & 92428-01-04-01 & 54143.95 &IS&     4.24(1) &     1.26(1) &     0.52(1) &    -0.35(1) &    0.265(7) &       22(1) &       87(14) &    1.336(3) &     1.08 \\
 & 92428-01-04-02 & 54144.09 &IS&     4.13(2) &     1.29(1) &     0.57(1) &    -0.23(1) &    0.230(5) &       22(3) &      125(46) &    1.361(3) &     0.97 \\
 & 92428-01-04-03 & 54144.87 &IS&     5.00(2) &     1.35(1) &     0.59(1) &    -0.33(1) &    0.253(5) &       25(3) &       81(33) &    1.346(4) &     1.31 \\
 & 92428-01-04-04 & 54145.96 &IS&     5.63(2) &     1.39(1) &    0.597(9) &    -0.38(1) &    0.270(5) &       22(2) &       89(33) &    1.346(3) &     1.17 \\
 & 92035-01-03-05 & 54145.11 &IS&     5.80(2) &     1.35(1) &    0.554(8) &    -0.50(1) &    0.307(6) &       25(2) &       81(17) &    1.303(3) &     1.37 \\
 & 92035-01-03-06 & 54146.03 &IS&     5.55(2) &     1.36(1) &    0.601(8) &    -0.40(1) &    0.269(4) &       21(2) &      111(24) &    1.343(2) &     1.29 \\
 & 92035-01-04-00 & 54147.01 &IS&     6.67(2) &     1.53(1) &    0.626(7) &   -0.608(9) &    0.338(5) & - & - &    1.371(3) &     1.59 \\
 & 92035-01-04-01 & 54148.14 &IS& - &     1.26(3) &    0.796(7) &    -0.96(1) &    0.194(5) & - & - &    1.024(6) &     1.07 \\
 & 92035-01-04-02 & 54149.69 &HSS& - &     1.19(2) &    0.782(4) &   -1.104(8) &    0.193(4) & - & - &    0.963(6) &     1.27 \\
\hline
 & 92704-03-08-01 & 54227.61 &HSS& - &     1.06(9) &     0.47(1) &    -1.23(4) &    0.051(3) &- & -&   0.0941(8) &     0.89 \\
 & 92704-03-09-00 & 54228.39 &HSS& - &     1.14(8) &     0.46(1) &    -1.12(4) &    0.050(3) &- & -&    0.097(1) &     1.20 \\
 & 92704-03-09-01 & 54229.24 &HSS& - &     1.05(7) &    0.444(9) &    -1.34(3) &    0.057(4) &- & -&   0.0850(6) &     1.64 \\
 & 92704-03-09-02 & 54230.70 &HSS& - &     1.00(7) &    0.450(9) &    -1.24(3) &    0.052(3) &- & -&   0.0909(7) &     1.47 \\
 & 92704-03-10-00 & 54231.60 &HSS& - &     1.10(8) &     0.48(1) &    -1.06(4) &    0.047(3) &- & -&    0.109(1) &     1.15 \\
 & 92704-03-10-11 & 54232.66 &IS& - &     1.09(5) &     0.49(1) &    -0.99(3) &    0.043(2) &- & -&    0.113(1) &     1.15 \\
 & 92704-03-10-12 & 54233.57 &IS& - &     0.93(4) &     0.47(1) &    -0.97(2) &    0.040(2) &- & -&    0.109(1) &     1.54 \\
 & 92704-03-11-00 & 54234.84 &IS&     4.05(9) &     0.93(4) &     0.47(2) &    -0.50(4) &    0.026(2) &- & -&    0.133(3) &     0.86 \\
 & 92704-03-11-01 & 54235.79 &IS&     3.24(8) &     0.80(4) &     0.49(3) &    -0.39(5) &    0.020(2) &- & -&    0.136(3) &     1.05 \\
 & 92704-04-01-00 & 54236.37 &IS&     2.91(6) &     0.81(4) &     0.49(3) &    -0.26(6) &    0.017(2) &- & -&    0.137(3) &     0.68 \\
 & 92704-04-01-01 & 54236.45 &IS&      3.0(2) &     0.71(4) &     0.52(2) &    -0.34(4) &    0.018(1) &- & -&    0.139(2) &     1.03 \\
 & 92704-04-01-02 & 54236.51 &IS&     2.70(5) &     0.72(4) &     0.54(4) &    -0.21(5) &    0.016(1) &- & -&    0.142(3) &     1.00 \\
 & 92704-03-12-00 & 54236.59 &IS& - &     0.77(5) &     0.50(5) &    -0.19(7) &    0.016(2) &- & -&    0.141(5) &     1.13 \\
 & 92704-04-01-03 & 54237.29 &IS& - &     0.76(5) &     0.55(4) &    -0.15(5) &   0.0150(9) &- & -&    0.135(2) &     0.76 \\
 & 92704-04-01-04 & 54237.36 &IS&      2.9(1) &     0.75(5) &     0.53(3) &    -0.19(5) &    0.015(1) &- & -&    0.136(3) &     0.94 \\
 & 92704-04-01-05 & 54237.42 &LHS&      2.8(1) &     0.69(4) &     0.58(3) &    -0.16(4) &   0.0146(5) &- & -&    0.138(2) &     1.04 \\
 & 92704-03-12-01 & 54237.49 &IS&     2.75(6) &     0.71(4) &     0.54(3) &    -0.20(4) &   0.0153(7) &- & -&    0.136(3) &     1.35 \\
 & 92704-04-01-06 & 54237.68 &IS&     2.49(6) &     0.76(3) &     0.53(3) &    -0.10(4) &   0.0146(7) &- & -&    0.138(3) &     0.97 \\
 & 92704-03-13-00 & 54238.74 &LHS& - &     0.61(5) &     0.58(6) &     0.06(7) &   0.0120(6) &- & -&    0.144(2) &     0.74 \\
 & 92704-03-13-01 & 54239.73 &LHS& - &     0.55(4) &     0.62(5) &     0.18(5) &   0.0108(3) &- & -&    0.142(2) &     0.71 \\
 & 92704-03-13-02 & 54240.30 &LHS&     1.90(8) &     0.56(3) &     0.50(4) &    -0.03(7) &   0.0120(7) &- & -&    0.138(3) &     0.70 \\
 & 92704-03-14-00 & 54241.56 &LHS&     1.44(4) &     0.50(5) &     0.65(8) &     0.27(7) &   0.0092(4) &- & -&    0.128(3) &     0.79 \\
 & 92704-03-14-01 & 54242.87 &LHS&      1.2(1) &     0.47(3) &     0.58(5) &     0.24(6) &   0.0086(2) &- & -&    0.122(2) &     0.60 \\
 & 92704-03-14-03 & 54244.97 &LHS&     0.76(3) &     0.47(6) &     0.62(9) &     0.34(9) &   0.0072(4) &- & -&    0.106(4) &     0.77 \\
 & 92704-04-02-00 & 54245.75 &LHS& - &     0.42(2) &     0.53(4) &     0.13(7) &   0.0073(2) &- & -&    0.099(1) &     0.78 \\
 & 92704-04-02-02 & 54245.88 &LHS&     0.72(3) &     0.43(4) &     0.57(7) &      0.2(1) &   0.0068(3) &- & -&    0.099(3) &     0.73 \\
 & 92704-03-15-00 & 54246.86 &LHS&    0.070(3) &     0.45(4) &     0.60(9) &     0.39(9) &   0.0059(3) &- & -&    0.092(3) &     1.00 \\
 & 92704-03-16-00 & 54247.91 &LHS& - &     0.43(6) &      0.6(1) &      0.3(1) &   0.0055(4) &- & -&    0.084(3) &     0.71 \\
 & 92704-03-17-00 & 54248.82 &LHS& - &     0.40(6) &      0.6(1) &      0.3(1) &   0.0053(4) &- & -&    0.079(4) &     0.71 \\
 & 92704-03-18-00 & 54249.54 &LHS& - &     0.42(5) &     0.62(9) &     0.41(9) &   0.0048(3) &- & -&    0.074(3) &     0.58 \\
 & 92704-03-19-00 & 54250.71 &LHS& - &     0.40(5) &      0.5(1) &      0.3(1) &   0.0042(3) &- & -&    0.067(3) &     0.60 \\
 & 92704-04-02-01 & 54251.69 &LHS& - &     0.40(4) &     0.69(7) &     0.45(4) &   0.0040(2) &- & -&    0.060(2) &     0.58 \\
 & 92704-04-02-04 & 54251.84 &LHS& - &     0.43(5) &      0.5(1) &      0.4(1) &   0.0036(3) &- & -&    0.059(3) &     0.54 \\
 & 92704-03-20-00 & 54252.04 &LHS& - &     0.43(5) &      0.5(1) &      0.4(1) &   0.0036(3) &- & -&    0.059(3) &     0.54 \\
\hline

